A Novel Deep Neural Network for Trajectory Prediction in Automated Vehicles Using Velocity Vector Field

Anticipating the motion of other road users is crucial for automated driving systems (ADS), as it enables safe and informed downstream decision-making and motion planning. Unfortunately, contemporary learning-based approaches for motion prediction exhibit significant performance degradation as the prediction horizon increases or the observation window decreases. This paper proposes a novel technique for trajectory prediction that combines a data-driven learning-based method with a velocity vector field (VVF) generated from a nature-inspired concept, i.e., fluid flow dynamics. In this work, the vector field is incorporated as an additional input to a convolutional-recurrent deep neural network to help predict the most likely future trajectories given a sequence of bird's eye view scene representations. The performance of the proposed model is compared with state-of-the-art methods on the HighD dataset demonstrating that the VVF inclusion improves the prediction accuracy for both short and long-term (5~sec) time horizons. It is also shown that the accuracy remains consistent with decreasing observation windows which alleviates the requirement of a long history of past observations for accurate trajectory prediction. Source codes are available at: https://github.com/Amir-Samadi/VVF-TP.

==> tex/problem_definition.tex <==


The problem is defined as a trajectory prediction of a target vehicle in a planner drivable area i.e. $x$ and $y$ coordinate as a function of time. The input data is provided as BEV including position, velocity, and dimension of vehicles (rectangular), as well as road boundaries and lane marking data. Given the prediction horizon $t_p$ and time step $\delta t_p$, the predicted $X$ and $Y$ component of the trajectory $T$ are $p = \left\lfloor {{{{t_p}} \mathord{\left/ {\vphantom {{{t_p}} {\delta t}}} \right. \kern-\nulldelimiterspace}{\delta t}_p}} \right\rfloor$ size vectors. Moreover, it is assumed that an observation of past trajectory over a certain period of time $t_o$ (discretized with ${\delta {t_o}}$ step) is also available for the prediction task. Therefore the observation and prediction length for a trajectory are $o = \left\lfloor {{{{t_o}} \mathord{\left/{\vphantom {{{t_o}} {\delta {t_o}}}} \right.\kern-\nulldelimiterspace} {\delta {t_o}}}} \right\rfloor$ and $p$, respectively, and they are mentioned as subscription and superscription for each trajectory $T_o^p = \left \{ {X_o^p,Y_o^p} \right\}$. Accordingly, the future location of the target vehicle, predicted with observation and prediction length of $o$ and $p$ at timestep $k \in \left\{ {1,2, \ldots ,p} \right\}$ is $\left[ {x\left( k \right),y\left( k \right)} \right]_o^p$. In addition, we assume that the drivable area (roads) and lane marking information is also given along with the nominal speed of the roads. Finally, since we consider BEV as the input data, occlusion with respect to the EV location has been ignored.
